Long-Lived LoRa: Prolonging the Lifetime of a LoRa Network

Prolonging the network lifetime is a major consideration in many Internet of Things applications. In this paper, we study maximizing the network lifetime of an energy-harvesting LoRa network. Such a network is characterized by heterogeneous recharging capabilities across the nodes that is not taken into account in existing work. We propose a link-layer protocol to achieve a long-lived LoRa network which dynamically enables the nodes with depleting batteries to exploit the superfluous energy of the neighboring nodes with affluent batteries by letting a depleting node offload its packets to an affluent node. By exploiting the LoRa's capability of adjusting multiple transmission parameters, we enable low-cost offloading by depleting nodes instead of high-cost direct forwarding. Such offloading requires synchronization of wake-up times as well as transmission parameters between the two nodes which also need to be selected dynamically. The proposed protocol addresses these challenges and prolongs the lifetime of a LoRa network through three novel techniques. (1) We propose a lightweight medium access control protocol for peer-to-peer communication to enable packet offloading which circumvents the synchronization overhead between the two nodes. (2) We propose an intuitive heuristic method for effective parameter selections for different modes (conventional vs. offloading). (3) We analyze the energy overhead of offloading and, based on it, the protocol dynamically selects affluent and depleting nodes while ensuring that an affluent node is not overwhelmed by the depleting ones. Simulations in NS-3 as well as real experiments show that our protocol can increase the network lifetime up to $4$ times while maintaining the same throughput compared to traditional LoRa network.

==> OffloadingOverview.tex <==
%!TEX root = main.tex


\section{Lading and Offloading Node Selection}

%section to describe and define lading and offloading nodes
\subsection{Transmission Count Prediction}

In order to correctly choose lading and offloading nodes, the gateway needs to estimate the total energy consumption of each node in the network. The total number of transmissions from each node is essential to compute its energy consumption in the conventional mode. Unfortunately, the unreliability in wireless networks makes it prohibitively difficult to predict the number of transmissions each node will make before the packet has been successfully received at the gateway. 

In case of failure to receive the packet at the gateway, a LoRa-WAN node can re-transmit a packet up to $8$ times. Thus, considering a fixed number of re-transmission overhead for every packet can introduce significant pessimism in estimating the total energy consumption of nodes. Consequently, it can lead to poor choices in lading and offloading node selection. 
 
%%Prediction algorithms 
To overcome this, we propose to use a prediction algorithm which determines the expected number of transmissions from each node in the network. Various machine learning techniques have been proposed to accurately predict the wireless network traffic in literature. Examples include the Autoregressive moving integrated average technique (ARIMA), Seasonal ARIMA~\cite{SARIMA}, Support Vector Machines, Multi-layer perception,~\cite{MLP} Gaussian Process and Long Short Term Memory (LSTM) architecture~\cite{LSTM}.

%%why we use LSTM
LSTM's are well equipped to determine the dependencies between events separated by a long time interval and provide an accurate prediction. We will use a LSTM network to predict the total number of transmissions from each node in the network. 
 %%Need more justification here

%%stucture of LSTM
LSTM is an recurrent neural network (RNN) architecture that recognizes long-term dependencies. While conventional RNN architectures suffer from the artifacts of exploding and vanishing gradient problems, LSTM's overcome this with the help of  memory cells which control the flow of information that passes through them to make a better prediction. 


Like other neural networks, LSTM networks consist of a chain of repeating LSTM blocks. Each block is usually called a memory cell consisting of three gates, which are the forget gate, the input gate and the output gate. Each gate takes three inputs, the current input $X_{t}$, the previous cell state $C_{t-1}$ and previous cell's output $h_{t-1}$.


The forget gate takes the current input and the previous cells output to determine which part of the input is irrelevant. This is then passed on to the input gate, which determines which part of the current cell state $C_{t}$ to update. Finally, the output gate decides the output of the block with the help of the new cell state provided by the input layer, the current input and the previous output. 

%%more details /equations about each gate here

%%Input and Output for LSTM
Our goal is to predict the total number of transmission attempts made by each node at time $t = T^l$. After each $T^l$ interval, we can reset $t$ to $0$. Thus, the input (usually called samples) to the LSTM network is the total transmission attempts made by each node at each packet reception time $t$. We assume that nodes will provide this information to the gateway in every packet they send. Thus, whenever a packet has been received at the gateway, a new sample is collected for the prediction. 

The LSTM network will predict for each node $V_i$ in the network the total number of transmission attempts to be made by $V_i$ at time $t= T^l$, denoted by $n^{tx}_{i}$. To train our LSTM network, we will let the nodes transmit to the gateway until we've received 1000 samples from each node. Then using this training data set, we can tune our hyper parameters such as window size, batch size and hidden neurons.  

%%LSTM Hyperparameters
The LSTM network can provide a prediction using various window-sizes. We could let the window size to incorporate every sample we've collected so far, or we could limit our window size to include samples from the last $w$ time steps. Using a large window size could become computationally expensive, whereas using a small window size could lead to prediction errors. 


Batch size is the number of samples that go through the LSTM network in a forward propagation, before a backward propagation happens. Selecting the correct batch size is important to prevent overfitting. 


The number of hidden neurons/ hidden LSTM layers influence the computational cost and the correctness of the output. Too many hidden layers can also lead to overfitting. 
%%more details about each hyperparameters could be discussed here after getting simulation results.


\subsection{Selection of Lading Nodes and Offloading Nodes}
After predicting the total number of transmission attempts for each node $V_i$ in the network, the gateway selects the lading and offloading nodes based on the amount of energy left in each node and the expected energy consumption. 

%%First algorithm to decide two sets offloading and lading

First we discuss how to select the offloading and lading nodes. The input to this algorithm is the set of all nodes in the network, $V$. For each node in $V_i$ in $V$ the gateway knows the estimated total number of transmission attempts $n_{tx}^{i}$ and the accumulated charge $B_i^*$ for node $V_i$.  The output of the algorithm will be two disjoint sets $\text{OFF}$ and $\text{L}$, representing offloading nodes and lading nodes respectively. 

Let us denote the energy consumption for node $V_i$ to transmit to the gateway as $E_{i}^{tx}$. Thus, we can estimate the total energy consumption for each node in conventional mode as $E^\text{conv}_{i} = n^{tx}_{i} \times E^\text{tx}_{i}$, for each $V_i \in V$. If $B_i^*>E^\text{conv}_{i}$, we will assign node $V_i$ to the set of lading nodes $L$ and compute its extra energy, $E^{x}_{i} = B_i^*-E^\text{conv}_i$. We can safely use $E^{x}_{i}$ to accommodate the lading mode.  If $B_i^*<=E^\text{conv}_{i}$ , we assign node $V_i$ to the set of offloading node $OFF$. 
%Then we can compute the number of transmissions node $i$ will fail to make as $n_{o}^{i}=\frac{E_{lag}^{i}}{E_{tx}^{i}}$. 
The process is described in Algorithm~\ref{alg:select_lading_offloading_1}


\begin{algorithm}[ht]
\caption{Selecting Lading and Offloading Nodes}\label{alg:select_lading_offloading_1}

\begin{algorithmic}
\STATE \textbf{Input:} Set of all nodes $V$  
\STATE \textbf{Output:} Disjoint sets $\text{OFF}, L$ 
\STATE $O \gets \emptyset$
\STATE $L \gets \emptyset$
\FOR {$V_i \in V$} 
        \STATE $E^\text{conv}_{i}  \gets n^{tx}_{i} \times E^{tx}_{i}$
        \IF {$E^\text{conv}_{i} < B_i^*$}
                \STATE $L \gets L \cup V_i$
        \ELSE 
                \STATE $\text{OFF} \gets \text{OFF} \cup V_i$
        \ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}

We represent the minimum energy consumption required for the offloading node $j$ to offload one packet to lading node $V_i$ as $E^\text{OFF}_{i,j}$. 
%We denote the minimum energy consumption required for the lading node $i$ to receive one packet from offloading node $j$  by $E_{cad}$. Note that, $E_{cad}$ depends only on the spreading factor and bandwidth used by the offloading node. As we are going to use a specific spreading factor (Lowest spreading factor) to enable the offload, we can consider this value is fixed and does not change with the offloaded packet. Thus, We can define the total energy overhead for lading node $i$ for accommodating the lading mode for one packet as $E_{lading}^{i}= E_{cad}+E_{tx}^{i}$. 



==> identification.tex <==
\section{Identifying Affluent and Starving Nodes}
\label{sec:identification}
